C3P: Contrastive promoter-protein pretraining yields representations capturing bacterial gene regulation

Despite the increasing scale of genome language models (gLMs), their ability to decode the function of regulatory sequences remains unclear. gLM pretraining relies on sequence reconstruction, which may struggle due to the noisy, rapidly evolving nature of regulatory DNA. Self-supervised contrastive approaches provide a promising alternative. Inspired by language-image architectures like CLIP, we introduce contrastive promoter-protein pretraining (C3P). By learning to align promoters to their corresponding proteins, we leverage the rich representations of proteins learned by protein language models as supervisory signal for the learning of promoter representations. After training on 88 million bacterial promoter-protein pairs, we evaluate the predictive power of C3P-learned promoter representations for inference of curated regulatory annotations, finding multi-fold improvement over leading gLMs. We also introduce zero-shot co-regulated gene retrieval, the ability to find co-regulated genes in a genome using no experimental data. We find that compared to a randomly initialized baseline, C3P training consistently provides significant zero-shot performance gains, unlike gLMs. Scaling analysis reveals the potential for further improvement as well as the efficiency of C3P, which achieved strong performance at a fraction of the training cost of leading gLMs. In addition to demonstrating that C3P training is effective for learning representations of bacterial regulatory sequences, our strong zero-shot co-regulated gene retrieval performance suggests the possibility of decoding gene regulation for millions of bacteria from their genomes alone.

==> sections/data_and_code_availability.tex <==
\section*{Data and Code Availability}

All data used in this work was sourced from publicly available databases. Codes for downloading data, extracting promoter protein pairs, and training C3P models are available at \href{https://github.com/dufaultc/contrastive-promoter-protein-pretraining}{https://github.com/dufaultc/contrastive-promoter-protein-pretraining}. Trained models available at \href{https://huggingface.co/dufaultc/contrastive-promoter-protein-pretraining}{https://huggingface.co/dufaultc/contrastive-promoter-protein-pretraining}.

